Simultaneously Updating All Persistence Values in Reinforcement Learning

In reinforcement learning, the performance of learning agents is highly sensitive to the choice of time discretization. Agents acting at high frequencies have the best control opportunities, along with some drawbacks, such as possible inefficient exploration and vanishing of the action advantages. The repetition of the actions, i.e., action persistence, comes into help, as it allows the agent to visit wider regions of the state space and improve the estimation of the action effects. In this work, we derive a novel All-Persistence Bellman Operator, which allows an effective use of both the low-persistence experience, by decomposition into sub-transition, and the high-persistence experience, thanks to the introduction of a suitable bootstrap procedure. In this way, we employ transitions collected at any time scale to update simultaneously the action values of the considered persistence set. We prove the contraction property of the All-Persistence Bellman Operator and, based on it, we extend classic Q-learning and DQN. After providing a study on the effects of persistence, we experimentally evaluate our approach in both tabular contexts and more challenging frameworks, including some Atari games.

==> algos/update.tex <==
\begin{algorithm}[t]
\medmuskip=0mu
\thinmuskip=0mu
\thickmuskip=0mu
\caption{All Persistence Bellman Update} \label{alg:pers_update}
\small
\begin{algorithmic}[1]
\REQUIRE Sampling persistence $\ksamp_t$, partial history $H_{t}^{\ksamp_t}$,\\ Q-function $Q$.%, step $t$.
\ENSURE Updated $Q$-function $Q'$
\vspace{0.1cm}
\STATE{$Q' \leftarrow Q$}
\FOR{$j=\ksamp_t, \ksamp_t-1 \dots, 1$}
%\STATE{$\tilde{\tau}_i \leftarrow ()$}
\FOR{$i=j-1, j-2,\dots, 0$}
\STATE{$k \leftarrow j-i$}
\STATE{\textcolor{vibrantMagenta}{$Q'(s_{t+i}, a_t, k) \leftarrow (1-\alpha)Q(s_{t+i}, a_t, k) +$}}
\STATE{\textcolor{vibrantMagenta}{$\quad \quad \quad \quad \quad \quad \quad \quad \alpha\widehat{T}^{\star}_{t+i} Q(s_{t+i}, a_t, k)$}}
%sample\_update(t+i, a, k)
\FOR{$d=1, 2,\dots, K_{\max}-k$}
\STATE{\textcolor{vibrantBlue}{$Q'(s_{t+i}, a_t, k+d) \leftarrow (1-\alpha)Q(s_{t+i}, a_t, k+d) +$}} % bootstrap\_update(t+i, a, k, d)
\STATE{\textcolor{vibrantBlue}{$\quad \quad \quad \quad \quad \quad \quad \quad \alpha{\widehat{T}}^{k}_{t+i} Q(s_{t+i}, a_t, k+d)$}}
\ENDFOR
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> plot_style.tex <==
%\usepakage{xcolor}

\definecolor{brightBlue}{RGB}{68, 119, 170}
\definecolor{brightCyan}{RGB}{102, 204, 238}
\definecolor{brightGreen}{RGB}{34, 136, 51}
\definecolor{brightYellow}{RGB}{204, 187, 68}
\definecolor{brightRed}{RGB}{238, 102, 119}
\definecolor{brightPurple}{RGB}{170, 51, 119}
\definecolor{brightGrey}{RGB}{187, 187, 187}

\definecolor{vibrantBlue}{RGB}{0, 119, 187}
\definecolor{vibrantMagenta}{RGB}{238, 51, 119}
\definecolor{vibrantTeal}{RGB}{0, 153, 136}
\definecolor{vibrantOrange}{RGB}{238, 119, 51}
\definecolor{vibrantCyan}{RGB}{51, 187, 238}
\definecolor{vibrantRed}{RGB}{204, 51, 17}

\definecolor{vibrantGrey}{RGB}{100, 100, 100}

\tikzstyle{dotted}=                  [dash pattern=on \pgflinewidth off 2pt]
\tikzstyle{densely dotted}=          [dash pattern=on \pgflinewidth off 1pt]
\tikzstyle{loosely dotted}=          [dash pattern=on \pgflinewidth off 4pt]

\tikzstyle{dashed}=                  [dash pattern=on 3pt off 3pt]
\tikzstyle{densely dashed}=          [dash pattern=on 3pt off 2pt]
\tikzstyle{very densely dashed}=          [dash pattern=on 4pt off 1pt]
\tikzstyle{loosely dashed}=          [dash pattern=on 3pt off 6pt]

\tikzstyle{dashdotted}=              [dash pattern=on 3pt off 2pt on \pgflinewidth off 2pt]
\tikzstyle{densely dashdotted}=      [dash pattern=on 3pt off 1pt on \pgflinewidth off 1pt]
\tikzstyle{loosely dashdotted}=      [dash pattern=on 3pt off 4pt on \pgflinewidth off 4pt]

\tikzstyle{dash dot dot}=[dash pattern=on 3pt off 2pt on \pgflinewidth off 2pt on \pgflinewidth off 2pt]
\tikzstyle{densely dash dot dot}=[dash pattern=on 3pt off 1pt on \pgflinewidth off 1pt on \pgflinewidth off 1pt]
\tikzstyle{loosely dash dot dot}= [dash pattern=on 3pt off 4pt on \pgflinewidth off 4pt on \pgflinewidth off 4pt]

\tikzstyle{dash dash dot}=[dash pattern=on 3pt off 2pt on 3pt off 2pt on \pgflinewidth off 2pt]
\tikzstyle{densely dash dash dot}=[dash pattern=on 3pt off 1pt on 3pt off 1pt on \pgflinewidth off 1pt]
\tikzstyle{loosely dash dash dot}= [dash pattern=on 3pt off 4pt on 3pt off 4pt on \pgflinewidth off 4pt]

\tikzstyle{dash dash dot dot}=[dash pattern=on 3pt off 2pt on 3pt off 2pt on \pgflinewidth off 2pt on \pgflinewidth off 2pt]
\tikzstyle{densely dash dash dot dot}=[dash pattern=on 3pt off 1pt on 3pt off 1pt on \pgflinewidth off 1pt on \pgflinewidth off 1pt]
\tikzstyle{loosely dash dash dot dot}= [dash pattern=on 3pt off 4pt on 3pt off 4pt on \pgflinewidth off 4pt on \pgflinewidth off 4pt]

\pgfplotsset{
	cycle list/.define={vibrant}{
        vibrantOrange, densely dashdotted, mark repeat=250,every mark/.append style={solid, fill=vibrantOrange, scale=2}, mark=o\\
    	vibrantBlue, densely dashed, mark repeat=350, every mark/.append style={solid, fill=vibrantBlue, scale=2},mark=*\\
    	vibrantRed, solid, mark repeat=200,every mark/.append style={solid, fill=vibrantRed, scale=3}, mark=x\\
        vibrantGrey, densely dash dash dot dot, mark repeat=40,every mark/.append style={solid, fill=vibrantGrey, scale=2}, mark=square*\\
    	vibrantCyan, densely dash dot dot, mark repeat=45,every mark/.append style={solid, fill=vibrantCyan, scale=2}, mark=triangle*\\
        vibrantMagenta, densely dash dash dot, mark repeat=50,every mark/.append style={solid, fill=vibrantMagenta, scale=2}, mark=star\\
    	vibrantTeal, densely dotted, mark repeat=30, every mark/.append style={solid, fill=vibrantTeal, scale=1}, mark=o\\
        },
    }
    
    
\pgfplotsset{
	cycle list/.define={vibrant2}{
    	vibrantTeal, densely dotted, mark repeat=8, every mark/.append style={solid, fill=vibrantTeal}, mark=square*\\
    	vibrantOrange, densely dashdotted, mark repeat=60,every mark/.append style={solid, fill=vibrantOrange, scale=2}, mark=diamond*\\
        vibrantRed, densely dash dot dot, mark repeat=60,every mark/.append style={solid, fill=vibrantRed, scale=3}, mark=x\\
    	vibrantGrey,densely dashed, mark repeat=60,every mark/.append style={solid, fill=vibrantGrey, scale=1.5}, mark=triangle*\\
    	vibrantBlue, solid, mark repeat=60, every mark/.append style={solid, fill=vibrantBlue},mark=*\\  
    },
}

\pgfplotsset{
	cycle list/.define={vibrant3}{
	  vibrantTeal, densely dotted, mark repeat=30, every mark/.append style={solid, fill=vibrantTeal, scale=1}, mark=o\\
	  	  vibrantRed, solid, mark repeat=20,every mark/.append style={solid, fill=vibrantRed, scale=3}, mark=x\\
    	vibrantGrey,densely dashed, mark repeat=3,every mark/.append style={solid, fill=vibrantGrey, scale=1.5}, mark=triangle*\\
    	vibrantBlue,  solid, mark repeat=3, every mark/.append style={solid, fill=vibrantBlue},mark=*\\  
    },
}


\pgfplotsset{
	cycle list/.define={single}{
    	vibrantBlue, solid, mark repeat=8, every mark/.append style={solid, fill=vibrantBlue},mark=*\\
        },
    }
    
    

\pgfplotsset{
	cycle list/.define={vibrantexchanged}{
	    vibrantRed, solid, mark repeat=200,every mark/.append style={solid, fill=vibrantRed, scale=3}, mark=x\\
        vibrantOrange, densely dashdotted, mark repeat=250,every mark/.append style={solid, fill=vibrantOrange, scale=2}, mark=o\\
    	vibrantBlue, densely dashed, mark repeat=350, every mark/.append style={solid, fill=vibrantBlue, scale=2},mark=*\\
        vibrantGrey, densely dash dash dot dot, mark repeat=40,every mark/.append style={solid, fill=vibrantGrey, scale=2}, mark=square*\\
    	vibrantCyan, densely dash dot dot, mark repeat=45,every mark/.append style={solid, fill=vibrantCyan, scale=2}, mark=triangle*\\
        vibrantMagenta, densely dash dash dot, mark repeat=50,every mark/.append style={solid, fill=vibrantMagenta, scale=2}, mark=star\\
    	vibrantTeal, densely dotted, mark repeat=30, every mark/.append style={solid, fill=vibrantTeal, scale=1}, mark=o\\
        },
    }
    
